CASUAL: Conditional Support Alignment for Domain Adaptation with Label Shift

Unsupervised domain adaptation (UDA) refers to a domain adaptation framework in which a learning model is trained based on the labeled samples on the source domain and unlabeled ones in the target domain. The dominant existing methods in the field that rely on the classical covariate shift assumption to learn domain-invariant feature representation have yielded suboptimal performance under label distribution shift. In this paper, we propose a novel Conditional Adversarial SUpport ALignment (CASUAL) whose aim is to minimize the conditional symmetric support divergence between the source's and target domain's feature representation distributions, aiming at a more discriminative representation for the classification task. We also introduce a novel theoretical target risk bound, which justifies the merits of aligning the supports of conditional feature distributions compared to the existing marginal support alignment approach in the UDA settings. We then provide a complete training process for learning in which the objective optimization functions are precisely based on the proposed target risk bound. Our empirical results demonstrate that CASUAL outperforms other state-of-the-art methods on different UDA benchmark tasks under different label shift conditions.

==> figures/big_table_with_variance.tex <==

\begin{table}[htbp]
	% \begin{minipage}{\linewidth}
	% \vskip -0.1in
	\centering
	\caption{Per-class average accuracies on USPS$\to$MNIST. Bold and underscore denote the best and second-best methods respectively}
	% \label{table:usps2mnist}
 \label{table:usps2mnist_mean}
	% \scalebox{0.83}{%
	% \begin{threeparttable}{

	\resizebox{0.95\textwidth}{!}{
	% \renewcommand{\arraystretch}{1.1}

	\begin{tabular}{lcccccc}
		\toprule

		Algorithm                          & $\alpha =$ None            & $\alpha = 10.0 $           & $\alpha = 3.0$             & $\alpha = 1.0$             & $\alpha = 0.5$             & AVG                \\
		\midrule

		No DA                              & $73.9 \pm 2.4$             & $73.8 \pm 2.5$             & $73.5 \pm 2.2$             & $73.9 \pm 2.3$             & $73.8 \pm 2.3$             & $73.8$             \\
		\midrule

		DANN \citep{ganin2015unsupervised} & $97.8 \pm 1.1$             & $96.1 \pm 1.0$             & $89.6 \pm 2.0$             & $78.7 \pm 2.5$             & $71.0 \pm 3.3$             & $86.6$             \\
		CDAN \citep{long2018conditional}   & $97.9 \pm 0.2$             & $97.6 \pm 0.2$             & $93.2 \pm 1.9$             & $81.7 \pm 2.9$             & $68.4 \pm 3.8$             & $87.8$             \\
		VADA~\citep{shu2018dirt}           & $\mathbf{98.1} \pm 0.1$    & $\mathbf{98.1} \pm 0.1$    & $\underline{96.8} \pm 1.1$ & $84.9 \pm 2.5$             & $76.8 \pm 3.9$             & $90.9$             \\
		\midrule
		% MDD Implicit                       & $$              & $$               & $$             & $$             & $$             \\

		IWDAN~\citep{tachet2020domain}     & $97.5 \pm 2.5$             & $97.1 \pm 3.2$             & $90.4 \pm 4.2$             & $81.3 \pm 4.1$             & $73.3 \pm 4.5$             & $87.9$             \\
		IWCDAN~\citep{tachet2020domain}    & $97.8 \pm 2.3$             & $97.5 \pm 2.0$             & $91.4 \pm 3.1$             & $82.6 \pm 2.9$             & $73.8 \pm 3.6$             & $88.7$             \\
		sDANN~\citep{wu2019domain}         & $87.4 \pm 0.6$             & $90.7 \pm 0.7$             & $92.1 \pm 1.9$             & $89.4 \pm 2.2$             & $85.2 \pm 3.4$             & $89.0$             \\
		% fDANN~\citep{wu2019domain}         & $ \pm $                    & $ \pm $                    & $ \pm $                    & $ \pm $                    & $ \pm $                    & $$                 \\
		ASA~\citep{tong2022adversarial}    & $94.1 \pm 0.6$             & $93.7 \pm 0.8$             & $94.1 \pm 0.2$             & $\underline{90.8} \pm 2.2$ & $\underline{84.7} \pm 1.1$ & $\underline{91.5}$ \\
		PCT~\citep{tanwisuth2021prototype} & $97.4 \pm 0.2$             & $97.2 \pm 0.2$             & $94.3 \pm 3.6$             & $82.3 \pm 4.4$             & $71.8 \pm 4.8$             & $88.6$             \\
		SENTRY~\citep{prabhu2021sentry}    & $97.5 \pm 2.0$             & $91.5 \pm 1.8$             & $91.4 \pm 2.2$             & $84.7 \pm 2.5$             & $82.3 \pm 3.1$             & $89.5$             \\
		% COAL                               & $$              & $$               & $$             & $$             & $$             \\
		\midrule


		\algoname\ (Ours)                  & $\underline{98.0} \pm 0.1$ & $\underline{98.0} \pm 0.2$ & $\textbf{97.2} \pm 0.5$    & $\textbf{96.7} \pm 0.6$    & $\textbf{88.3} \pm 1.7$    & $\textbf{95.6}$    \\

		% & $$              & $$               & $$             & $$             & $$             \\

		% \midrule


		\bottomrule
	\end{tabular}
	}

\end{table}

% \vskip -0.2in
\begin{table}[htbp]
	% \begin{minipage}{\linewidth}
	%\vskip -0.1in
	\centering
	\caption{Results on STL$\to$CIFAR. Same setup as Table \ref{table:usps2mnist_mean}}
	% \label{table:stl2cifar}
 \label{table:stl2cifar_mean}
	% \scalebox{0.83}{%
	% \begin{threeparttable}{

	\resizebox{0.9\textwidth}{!}{
	% \renewcommand{\arraystretch}{1.1}

	\begin{tabular}{lcccccc}
		\toprule

		% & \multicolumn{2}{c}{$\alpha = 0.0$}                                                    & \multicolumn{2}{c}{$\alpha = 1.0$}                                                    & \multicolumn{2}{c}{$\alpha = 1.5$}                                                    & \multicolumn{2}{c}{$\alpha = 2.0$} \\
		% \cmidrule(lr){2-3}
		% \cmidrule(lr){4-5}
		% \cmidrule(lr){6-7}
		% \cmidrule(lr){8-9}
		% Algorithm & \multicolumn{1}{c}{average} & \multicolumn{1}{c}{min} & \multicolumn{1}{c}{average} & \multicolumn{1}{c}{min} & \multicolumn{1}{c}{average} & \multicolumn{1}{c}{min} & \multicolumn{1}{c}{average} & \multicolumn{1}{c}{min} \\

		Algorithm                          & $\alpha =$ None            & $\alpha = 10.0 $           & $\alpha = 3.0$             & $\alpha = 1.0$             & $\alpha = 0.5$             & AVG                \\
		\midrule

		No DA                              & $69.9 \pm 0.6$             & $69.8 \pm 0.7$             & $69.7 \pm 0.3$             & $68.8 \pm 0.9$             & $67.9 \pm 1.0$             & $69.2$             \\
		\midrule

		DANN \citep{ganin2015unsupervised} & $75.3 \pm 0.3$             & $74.3 \pm 0.4$             & $73.5 \pm 0.8$             & $70.0 \pm 2.1$             & $67.1 \pm 3.0$             & $72.0$             \\
		CDAN \citep{long2018conditional}   & $75.5 \pm 0.3$             & $74.1 \pm 0.3$             & $73.5 \pm 0.3$             & $71.3 \pm 1.7$             & $67.6 \pm 2.9$             & $72.4$             \\
		VADA~\citep{shu2018dirt}           & $\mathbf{77.1} \pm 0.3$    & $75.5 \pm 0.4$             & $73.8 \pm 0.7$             & $71.3 \pm 1.5$             & $68.0 \pm 1.0$             & $73.1$             \\
		\midrule
		% MDD Implicit                       & $$              & $$               & $$             & $$             & $$             \\

		IWDAN~\citep{tachet2020domain}     & $72.9 \pm 0.8$             & $72.6 \pm 1.0$             & $71.8 \pm 0.9$             & $70.6 \pm 1.0$             & $69.5 \pm 1.1$             & $71.5$             \\
		IWCDAN~\citep{tachet2020domain}    & $72.1 \pm 1.0$             & $72.0 \pm 0.4$             & $71.5 \pm 0.5$             & $71.9 \pm 0.7$             & $69.9 \pm 0.9$             & $71.5$             \\
		sDANN~\citep{wu2019domain}         & $72.8 \pm 0.4$             & $72.0 \pm 0.3$             & $72.0 \pm 0.8$             & $71.4 \pm 1.1$             & $\underline{70.1} \pm 0.9$ & $71.7$             \\
		% fDANN~\citep{wu2019domain}         & $ \pm $                    & $ \pm $                    & $ \pm $                    & $ \pm $                    & $ \pm $                    & $$                 \\
		ASA~\citep{tong2022adversarial}    & $72.7 \pm 0.4$             & $72.2 \pm 0.5$             & $72.1 \pm 0.8$             & $\underline{71.5} \pm 1.0$ & $69.8 \pm 0.7$             & $71.7$             \\
		PCT~\citep{tanwisuth2021prototype} & $75.0 \pm 0.2$             & $76.1 \pm 0.2$             & $75.0 \pm 0.9$             & $70.9 \pm 1.6$             & $68.3 \pm 2.3$             & $73.1$             \\
		SENTRY~\citep{prabhu2021sentry}    & $76.7 \pm 0.5$             & $\underline{76.6} \pm 1.3$ & $\underline{75.2} \pm 1.2$ & $71.2 \pm 1.0$             & $67.0 \pm 1.6$             & $\underline{73.3}$ \\
		\midrule
		\algoname\ (Ours)                  & $\underline{76.9} \pm 0.6$ & $\mathbf{76.8} \pm 0.6$    & $\mathbf{75.8} \pm 0.5$    & $\mathbf{74.2} \pm 1.1$    & $\mathbf{71.7} \pm 1.2$    & $\textbf{75.1}$    \\

		% & $$              & $$               & $$             & $$             & $$             \\

		% \midrule


		\bottomrule
	\end{tabular}
	}
\end{table}

\begin{table}[htbp]
	% \begin{minipage}{\linewidth}
	% \vskip -0.1in
	\centering
	\caption{Results on VisDA-2017. Same setup as Table \ref{table:usps2mnist_mean}}
	% \label{table:visda17}
 \label{table:visda17_mean}
	% \scalebox{0.83}{%
	% \begin{threeparttable}{

	\resizebox{0.9\textwidth}{!}{
	% \renewcommand{\arraystretch}{1.1}

	\begin{tabular}{lcccccc}
		\toprule

		Algorithm                          & $\alpha =$ None            & $\alpha = 10.0 $           & $\alpha = 3.0$             & $\alpha = 1.0$             & $\alpha = 0.5$             & AVG                \\
		\midrule

		No DA                              & $55.6 \pm 0.7$             & $56.0 \pm 0.7$             & $55.5 \pm 0.8$             & $55.2 \pm 0.9$             & $55.1 \pm 0.8$             & $55.5$             \\
		\midrule

		DANN \citep{ganin2015unsupervised} & $\textbf{75.5} \pm 0.4$    & $71.3 \pm 0.4$             & $68.4 \pm 1.8$             & $62.2 \pm 2.2$             & $56.4 \pm 1.6 $            & $66.8$             \\
		CDAN \citep{long2018conditional}   & $75.0 \pm 0.3$             & $72.5 \pm 0.4$             & $69.8 \pm 2.8$             & $61.3 \pm 2.9$             & $56.3 \pm 3.1 $            & $67.0$             \\
		VADA~\citep{shu2018dirt}           & $\underline{75.2} \pm 0.9$ & $72.3 \pm 1.2$             & $69.6 \pm 1.6$             & $59.2 \pm 1.8$             & $52.6 \pm 2.3$             & $65.8$             \\
		\midrule
		% MDD Implicit                       & $$              & $$               & $$             & $$             & $$             \\

		IWDAN~\citep{tachet2020domain}     & $74.1 \pm 0.9$             & $\underline{73.3} \pm 0.9$    & $\underline{71.4} \pm 1.1$ & $65.3 \pm 2.3$             & $59.7 \pm 2.6$             & $\underline{68.8}$ \\
		IWCDAN~\citep{tachet2020domain}    & $73.5 \pm 1.1$             & $72.5 \pm 0.4$             & $69.6 \pm 1.9$             & $62.9 \pm 2.8$             & $57.2 \pm 3.4$             & $67.1$             \\
		sDANN~\citep{wu2019domain}         & $72.8 \pm 1.1$             & $72.2 \pm 1.1$             & $71.2 \pm 2.3$             & $\underline{64.9} \pm 3.3$ & $\underline{62.5} \pm 3.1$ & $68.7$             \\
		% fDANN~\citep{wu2019domain}         & $ \pm $                    & $ \pm $                    & $ \pm $                    & $ \pm $                    & $ \pm $                    & $$                 \\
		ASA~\citep{tong2022adversarial}    & $66.4 \pm 0.3$             & $65.3 \pm 1.3$             & $64.6 \pm 2.1$             & $61.7 \pm 2.8$             & $60.1 \pm 2.0$             & $63.6$             \\
		PCT~\citep{tanwisuth2021prototype} & $68.2 \pm 2.3$             & $66.8 \pm 2.9$             & $65.4 \pm 3.1$             & $60.5 \pm 3.6$             & $53.6 \pm 3.9$             & $63.3$             \\
		SENTRY~\citep{prabhu2021sentry}    & $67.5 \pm 0.5$             & $64.5 \pm 1.5$             & $57.6 \pm 1.7$             & $53.4 \pm 3.2$             & $52.6 \pm 3.6$             & $59.1$             \\
		\midrule


		\algoname\ (Ours)                  & $74.3 \pm 1.5$             & $\textbf{73.4} \pm 1.3$ & $\textbf{71.8} \pm 1.3$    & $\textbf{66.3} \pm 2.3$    & $\textbf{63.2} \pm 2.5$    & $\textbf{69.8}$    \\

		% & $$              & $$               & $$             & $$             & $$             \\

		% \midrule


		\bottomrule
	\end{tabular}
	}

\end{table}


% \vskip -0.1in
\begin{table}[htbp]
	% \begin{minipage}{\linewidth}
	%\vskip -0.1in
	\centering
	\caption{Ablation study of individual loss terms}
	\label{table:ablation1}
	% \scalebox{0.83}{%
	% \begin{threeparttable}{

	% \resizebox{0.9\textwidth}{!}{
	% \renewcommand{\arraystretch}{1.1}

	\begin{tabular}{ccc|cccccc}
		\toprule

		$\mathcal{L}_{align}$ & $\mathcal{L}_{ce}$ & $\mathcal{L}_{v}$ & $\alpha =$ None & $\alpha = 10.0 $ & $\alpha = 3.0$ & $\alpha = 1.0$ & $\alpha = 0.5$ & AVG    \\ \hline

		$\checkmark$          & $$                 & $$                & $94.5$          & $94.2$           & $94.3$         & $94.3$         & $84.9$         & $92.4$ \\
		% $\checkmark$          & $$                 & $\checkmark$      & $95.3$              & $$               & $$             & $$             & $74.1$             & $$     \\
		$\checkmark$          & $\checkmark$       & ${}$                & $97.7$          & $97.2$           & $96.8$         & $96.2$         & $87.4$         & $95.1$ \\
		$\checkmark$          & $\checkmark$       & $\checkmark$      & $\textbf{98.0}$          & $\textbf{98.0}$           & $\textbf{97.2}$         & $\textbf{96.7}$         & $\textbf{88.3}$         & $\textbf{95.6}$ \\

		% \midrule


		\bottomrule
	\end{tabular}
	% }
\end{table}

==> figures/fig_lineplot_cssd.tex <==
\begin{figure*}[!htb]
	% \vskip -0.1in
	\centering
	% \newcommand\figvis{1.26in}

	\subfloat[Target accuracy during training]{\includegraphics[height=1.9in]{figures/Accuracy on target domain_upscaled.png}}
	\subfloat[CSSD during training]{\includegraphics[height=1.9in]{figures/CSSD distance_upscaled.png}}

	\caption{\textit{Left} Accuracy of various algorithms during training. \textit{Right} Computed CSSD (Eq. \ref{def:cssd}) for learned feature.}
	  % The plots correspond to averages over 5 independent runs.}
	  % Similar to Figure \ref{fig:vis_2d}, the label probabilities are equal in the source domain, while they are [22.9\%, 64.7\%, 12.4\%] in the target domain.}
	% $\mathcal{D}_W$ and $\mathcal{D}_\triangle$ between embeddings.
	\label{fig:cssd_line_plot}
 \vskip -0.3cm
\end{figure*}


==> figures/fig_vis_feature2d.tex <==
\captionsetup[subfloat]{justification=centering}
\begin{figure*}[!htbp]
	%\vskip -0.1in
	\centering
	\newcommand\figvis{1.26in}
	% \subfloat[No DA (avg acc: $63 \%$)\\$\mathcal{D}_W(p^\theta_Z, q^\theta_Z) = 0.78$ \\ $\mathcal{D}_\triangle(p^\theta_Z, q^\theta_Z) =  0.10$]{\includegraphics[height=\figvis]{figures/vis2d_no_da.pdf}}\quad
	% \subfloat[DANN (avg acc: $75 \%$)\\$\mathcal{D}_W(p^\theta_Z, q^\theta_Z) = 0.07$ \\ $\mathcal{D}_\triangle(p^\theta_Z, q^\theta_Z) =  0.02$]{\includegraphics[height=\figvis]{figures/vis2d_dann.pdf}}\quad
	% \subfloat[No DA (avg acc: $63 \%$)]{\includegraphics[height=\figvis]{figures/vis2d_no_da.pdf}}
	\subfloat[CDAN (avg acc: $85 \%$)\\$\mathcal{D}_W=0.14$ \\$\mathcal{D}^c_{\supp}=0.13$]{\includegraphics[height=\figvis]{figures/vis2d_cdan.pdf}}
	\subfloat[ASA (avg acc: $93 \%$)\\$\mathcal{D}_W=0.63$ \\$\mathcal{D}^c_{\supp}=0.05$]{\includegraphics[height=\figvis]{figures/vis2d_asa.pdf}}
	\subfloat[\algoname (avg acc: $99 \%$)\\$\mathcal{D}_W=0.65$ \\$\mathcal{D}^c_{\supp}=0.02$]{\includegraphics[height=\figvis]{figures/vis2d_casa.pdf}}
	\caption{Visualization of support of feature representations for 3 classes in the USPS $\to$ MNIST task.
	% Each panel shows 2 level sets (outer one approximates the support) of the kernel density estimates of embeddings in source (filled regions) and target domains (solid/dashed lines)..
	Each plot illustrates the 2 level sets of kernel density estimates for both the source and target features.
 % The average accuracy, Wasserstein distance $\mathcal{D}_W$ and $\mathcal{D}^c_{\supp}$ are also provided.
 }
	% $\mathcal{D}_W$ and $\mathcal{D}_\triangle$ between embeddings.
	\label{fig:vis_2d}
\end{figure*}


==> figures/tables.tex <==
\captionsetup{
	margin=8pt
}

\begin{table*}

    \begin{minipage}[h]{0.5\textwidth}

	\caption{\small Per-class average accuracies on USPS$\to$MNIST.}
	\label{table:usps2mnist_mean}
	\scalebox{0.85}{
		\begin{tabular}{lcccccc}
   & \multicolumn{5}{c}{$\alpha$} & \\ \cline{2-6}
   Algorithm         & $\emptyset$ & $10$ & $3$ & $1$ & $0.5$ & {Average} \\ \midrule
			% Algorithm         & \rotatebox{90}{$\alpha =$ None} & \rotatebox{90}{$\alpha=10$} & \rotatebox{90}{$\alpha=3.0$} & \rotatebox{90}{$\alpha=1.0$} & \rotatebox{90}{$\alpha=0.5$} & \rotatebox{90}{Average} \\ \midrule

			No DA             & $73.9$                          & $73.8$                      & $73.5$                       & $73.9$                       & $73.8$                       & $73.8$                  \\	\midrule

			% 	DANN  & $97.8$             & $96.1$             & $89.6$             & $78.7$             & $71.0$             & $86.6$             \\
			% CDAN    & $97.9$             & $97.6$             & $93.2$             & $81.7$             & $68.4$             & $87.8$             \\
			DANN*             & $96.2$                          & $96.2$                      & $93.5$                       & $82.6$                       & $72.3$                       & $88.2$                  \\
			CDAN*             & $96.6$                          & $96.5$                      & $93.7$                       & $82.2$                       & $70.7$                       & $88.0$                  \\

			VADA~             & $\mathbf{98.1}$                 & $\mathbf{98.1}$             & $\underline{96.8}$           & $84.9$                       & $76.8$                       & $90.9$                  \\
			SDAT              & $97.8$                          & $97.5$                      & $94.1$                       & $83.3$                       & $68.8$                       & $88.3$                  \\
			MIC               & $\underline{98.0}$              & $97.6$                      & $95.2$                       & $82.9$                       & $70.8$                       & $88.9$                  \\
			DALN & $97.2$ & $96.3$ & $91.2$ & $83.4$ & $72.5$ & $88.2$ \\                                                                              
			\midrule
			% MDD Implicit                       & $$              & $$               & $$             & $$             & $$             \\

			IWDAN~            & $97.5$                          & $97.1$                      & $90.4$                       & $81.3$                       & $73.3$                       & $87.9$                  \\
			IWCDAN~           & $97.8$                          & $97.5$                      & $91.4$                       & $82.6$                       & $73.8$                       & $88.7$                  \\
			sDANN~            & $87.4$                          & $90.7$                      & $92.1$                       & $89.4$                       & $85.2$                       & $89.0$                  \\
			ASA~              & $94.1$                          & $93.7$                      & $94.1$                       & $90.8$           & $84.7$           & $91.5$      \\
			PCT~              & $97.4$                          & $97.2$                      & $94.3$                       & $82.3$                       & $71.8$                       & $88.6$                  \\
			SENTRY~           & $97.5$                          & $91.5$                      & $91.4$                       & $84.7$                       & $82.3$                       & $89.5$                  \\
			OSTAR & $97.7$ & $97.6$ & $95.7$ & $\underline{91.3}$ & $\underline{84.7}$ & $\underline{93.4}$ \\
BIWAA & $97.5$ & $97.5$ & $91.6$ & $82.7$ & $73.3$ & $88.6$ \\
MARS & $96.8$ & $92.6$ & $88.5$ & $85.3$ & $83.5$ & $89.4$ \\
                                                             
			\midrule


			\algoname\ (Ours) & $\underline{98.0}$              & $\underline{98.0}$          & $\textbf{97.2}$              & $\textbf{96.7}$              & $\textbf{88.3}$              & $\textbf{95.6}$         \\
		\end{tabular}
	}
     \end{minipage}
\begin{minipage}[h]{0.5\textwidth}
% \end{table}

% \begin{table}[!htbp]

 % \caption{\small Per-class accuracy on STL$\to$CIFAR. Same setup as Table \ref{table:usps2mnist_mean}.}
 \caption{\small Per-class average accuracies on STL$\to$CIFAR.}
	\label{table:stl2cifar_mean}
	\scalebox{0.85}{
		\begin{tabular}{lcccccc}
  & \multicolumn{5}{c}{$\alpha$} & \\ \cline{2-6}
   Algorithm         & $\emptyset$ & $10$ & $3$ & $1$ & $0.5$ & {Average} \\ \midrule
			% Algorithm         & \rotatebox{90}{$\alpha =$ None} & \rotatebox{90}{$\alpha=10$} & \rotatebox{90}{$\alpha=3.0$} & \rotatebox{90}{$\alpha=1.0$} & \rotatebox{90}{$\alpha=0.5$} & \rotatebox{90}{Average} \\
			% \midrule

			No DA             & $69.9$                          & $69.8$                      & $69.7$                       & $68.8$                       & $67.9$                       & $69.2$                  \\
			\midrule

			% DANN              & $75.3$                          & $74.3$                      & $73.5$                       & $70.0$                       & $67.1$                       & $72.0$                  \\
			% CDAN              & $75.5$                          & $74.1$                      & $73.5$                       & $71.3$                       & $67.6$                       & $72.4$                  \\
			DANN*             & $75.9$                          & $74.9$                      & $74.1$                       & $71.7$                       & $69.5$                       & $\underline{73.2}$      \\
			CDAN*             & $75.6$                          & $74.3$                      & $73.7$                       & $71.8$           & $69.7$           & $73.0$                  \\

			VADA~             & $\mathbf{77.1}$                 & $75.5$                      & $73.8$                       & $71.3$                       & $68.0$                       & $73.1$                  \\
			SDAT              & $75.8$                          & $74.4$                      & $71.5$                       & $68.3$                       & $66.2$                       & $71.2$                  \\
			MIC               & $76.4$                          & $75.5$                      & $72.7$                       & $68.6$                       & $67.3$                       & $72.1$                  \\
		DALN & $74.3$ & $74.1$ & $72.8$ & $70.3$ & $68.4$ & $72.0$ \\

			\midrule
			% MDD Implicit                       & $$              & $$               & $$             & $$             & $$             \\

			IWDAN~            & $72.9$                          & $72.6$                      & $71.8$                       & $70.6$                       & $69.5$                       & $71.5$                  \\
			IWCDAN~           & $72.1$                          & $72.0$                      & $71.5$                       & $\underline{71.9}$                       & $\underline{69.9}$                       & $71.5$                  \\
			sDANN~            & $72.8$                          & $72.0$                      & $72.0$                       & $71.4$                       & $70.1$                       & $71.7$                  \\
			ASA~              & $72.7$                          & $72.2$                      & $72.1$                       & $71.5$                       & $69.8$                       & $71.7$                  \\
			PCT~              & $75.0$                          & $76.1$                      & $75.0$                       & $70.9$                       & $68.3$                       & $73.1$                  \\
			SENTRY~           & $76.7$                          & $\underline{76.6}$          & $\underline{75.2}$           & $71.2$                       & $67.0$                       & $73.3$                  \\
			OSTAR & $73.7$ & $72.4$ & $70.8$ & $70.1$ & $68.4$ & $71.1$ \\
BIWAA & $75.7$ & $74.5$ & $72.1$ & $70.6$ & $66.3$ & $71.9$ \\
MARS & $72.8$ & $71.3$ & $69.7$ & $67.6$ & $65.9$ & $69.5$ \\

			\midrule
			\algoname\ (Ours) & $\underline{76.9}$              & $\mathbf{76.8}$             & $\mathbf{75.8}$              & $\mathbf{74.2}$              & $\mathbf{71.7}$              & $\textbf{75.1}$         \\
		\end{tabular}
	}
 \end{minipage}
\end{table*}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

